FedMood: Federated Learning on Mobile Health Data for Mood Detection

Depression is one of the most common mental illness problems, and the symptoms shown by patients are not consistent, making it difficult to diagnose in the process of clinical practice and pathological research. Although researchers hope that artificial intelligence can contribute to the diagnosis and treatment of depression, the traditional centralized machine learning needs to aggregate patient data, and the data privacy of patients with mental illness needs to be strictly confidential, which hinders machine learning algorithms clinical application. To solve the problem of privacy of the medical history of patients with depression, we implement federated learning to analyze and diagnose depression. First, we propose a general multi-view federated learning framework using multi-source data, which can extend any traditional machine learning model to support federated learning across different institutions or parties. Secondly, we adopt late fusion methods to solve the problem of inconsistent time series of multi-view data. Finally, we compare the federated framework with other cooperative learning frameworks in performance and discuss the related results.

==> 5-Relatedwork.tex <==
\section{Related Work}~\label{sec:relate}

In this section, we introduce the related research results of %depression,
federated learning and multi-view learning, and discuss the recently proposed federated multi-view learning.

\iffalse
\noindent\textbf{Depression.}According to statistics from the World Health Organization, depression has surpassed coronary heart disease as the world's second-largest disease affecting human health \cite{world2008global}. 
The clinical characteristics of patients with depression are mainly marked and lasting depression. 
Accompanied by depression, they will often go from initial depression to low self-esteem depression, and even pessimistic world-weariness, leading to suicidal behavior \cite{marcus2012depression}.
So far, people have not identified the cause of depression, but biological, psychological and social environmental factors are closely related to the onset of depression \cite{world2001world}. 
These factors make it difficult to diagnose depression, and it may be confused with the symptoms of other diseases \cite{alghowinem2015multimodal}. 
Many people who usually seem to be smiling and optimistic may be experiencing pain and suffering in their hearts. 
Most depression patients are not well diagnosed. 
In many countries, less than 10\% of patients can receive treatment, which may increase depression The impact of disease \cite{alibrahim2010gender,world2017depression}.
\fi

\noindent\textbf{Multi-View learning.} Xu et al. \cite{xu2013survey} pointed out that multi-perspective learning requires the use of one function to model one perspective and the use of other perspectives to jointly optimize all functions. Cao et al. \cite{cao2016multi,cao2014tensor} used tensor product to process multi-view data. 
Yao et al. \cite{yao2018deep} integrated CNN, LSTM and Graph embedding tackled the complex nonlinear spatial and temporal dependency in a multi-perspective way. In addition, some work integrates multi-view into the process of deep learning \cite{zhang2016identifying} and transfer learning \cite{wu2017online}, so as to help expand samples from data.

\noindent\textbf{Federated learning.} Here we mainly refer to the medical application of federated learning and some common federated multi-View deep learning framework.

\iffalse
Federated learning enables each medical institution to form a large data set on the premise of protecting the privacy of their patients, which can better conduct drug research and development, reduce the cost of medical diagnosis, medical image processing, genetic analysis, etc \cite{dash2019big,dua2014machine,li2019privacy,wagner2016privacy}. \fi

\iffalse
Kim Y et al. \cite{kim2017federated} used joint analysis of data from multiple hospitals to discover the phenotype of a specific patient population under the condition that no data left the local hospital. 
In the case of federated learning, the algorithm can find the "sickle cell/chronic pain" characterization that cannot be found in a hospital alone, avoiding deviations in the results due to population differences and small samples. 
\fi
Lee et al. \cite{lee2018privacy} proposed a privacy protection platform in the federated environment, which could find similar patients from different hospitals without sharing patient-level information. 
Huang L et al. \cite{huang2019patient} improved the performance of federated learning for predicting mortality and length of stay by using feature autoencoders and patient clustering. 
However, the method of combining federated learning and multi-view data in existing research is still in the development stage.
Adrian Flanagan et al. \cite{flanagan2020federated} proposed the federated multi-view matrix factorization method and address cold-start problem.
Huang et al. \cite{huang2020federated} proposed FL-MV-DSSM, which is the first general content-based joint multi-view framework, which successfully extended traditional federated learning to federated multi-view learning.
Kang et al. \cite{kang2020fedmvt} proposed the FedMVT algorithm for semi-supervised learning, which can improve the performance of vertical federated learning with limited overlapping samples.
These related methods using public datasets are mainly used to recommend systems to solve the cold start problem. 
However, our framework uses data collected from mobile devices to solve medical mood prediction problems.
\iffalse
Wenqi L et al. \cite{li2019privacy} used the $\epsilon$-differential privacy framework to improve the security of federated learning and protect the data privacy of patients and medical institutions. 
Liu et al. \cite{liu2019two} conducted a study on patient-representative learning and obesity comorbidity phenotype using federated learning with good results.
\fi


%In this section, we introduce XXXXX.
